From Lab to Wrist: Bridging Metabolic Monitoring and Consumer Wearables for Heart Rate and Oxygen Consumption Modeling

Understanding physiological responses during running is critical for performance optimization, tailored training prescriptions, and athlete health management. We introduce a comprehensive framework -- what we believe to be the first capable of predicting instantaneous oxygen consumption (VO$_{2}$) trajectories exclusively from consumer-grade wearable data. Our approach employs two complementary physiological models: (1) accurate modeling of heart rate (HR) dynamics via a physiologically constrained ordinary differential equation (ODE) and neural Kalman filter, trained on over 3 million HR observations, achieving 1-second interval predictions with mean absolute errors as low as 2.81\,bpm (correlation 0.87); and (2) leveraging the principles of precise HR modeling, a novel VO$_{2}$ prediction architecture requiring only the initial second of VO$_{2}$ data for calibration, enabling robust, sequence-to-sequence metabolic demand estimation. Despite relying solely on smartwatch and chest-strap data, our method achieves mean absolute percentage errors of approximately 13\%, effectively capturing rapid physiological transitions and steady-state conditions across diverse running intensities. Our synchronized dataset, complemented by blood lactate measurements, further lays the foundation for future noninvasive metabolic zone identification. By embedding physiological constraints within modern machine learning, this framework democratizes advanced metabolic monitoring, bridging laboratory-grade accuracy and everyday accessibility, thus empowering both elite athletes and recreational fitness enthusiasts.

==> Sections/5-0-RunnerSig.tex <==
Running dynamics describe a runner's form, efficiency, and performance through a range of measurable metrics. These metrics can be captured using specialized sensors or devices, such as Garmin watches, to provide runners with deeper insights into their running mechanics. Key variables in running dynamics include cadence, vertical oscillation, ground contact time, stride length, and more.

\textbf{Cadence}  
Cadence measures the number of steps a runner takes per minute. Trained runners typically exhibit cadences ranging from 170 to 180 steps per minute. A consistently lower cadence may indicate overstriding, a movement pattern that can lead to inefficiencies and increase the risk of injury. Overstriding can lower a runner’s running economy, as longer steps generally require more energy, leading to greater fatigue, reduced speed, and diminished endurance.

\textbf{Stance Time} (also referred to as ground contact time, or GCT) measures how long a runner's foot remains on the ground during each stride, typically expressed in milliseconds \cite{...}. Shorter stance times are generally associated with improved running efficiency and performance, as less ground contact implies that the runner spends less energy with each stride. Conversely, longer stance times may indicate excessive ground contact, potentially reducing running economy, increasing fatigue, and elevating the risk of injury. A longer stance time is also often linked with overstriding, where the foot lands ahead of the runner’s center of mass.

\textbf{Vertical Ratio}  
Vertical ratio quantifies the amount of vertical oscillation (up-and-down body movement) relative to stride length, typically represented as a percentage. A lower vertical ratio generally correlates with enhanced running efficiency and performance, as it suggests that a runner is minimizing wasted vertical motion and channeling more energy into forward propulsion \cite{...}. Conversely, a higher vertical ratio may indicate excessive energy expenditure on vertical movement, thereby diminishing running economy.

\textbf{Stance Time Balance}  
Stance time balance measures the symmetry between a runner’s left and right legs in terms of ground contact time per stride. Expressed as a percentage, it offers insights into a runner’s form and technique. A 50\% balance indicates equal ground contact time for both legs, while deviations from this value point to asymmetry. This asymmetry can arise from differences in leg strength, foot strike patterns, or running mechanics and may lead to uneven load distribution, increasing injury risk and reducing running efficiency.

\textbf{Step Length}  
Step length measures the distance covered between a runner’s steps, typically expressed in meters or feet. Longer strides are generally considered more efficient, as they allow the runner to cover more ground with each step, provided that a good cadence is maintained. This balance ensures optimal performance and efficiency during running.

In conclusion, running dynamics parameters offer valuable insights into a runner’s form, technique, and overall efficiency. By tracking and analyzing these metrics, runners can optimize their training, reduce injury risk, and enhance their performance outcomes. Here, we demonstrate the various effects of each of these parameters compared to the length of windows of sessions to differentiate between different runners. Across over 500 sessions of running workouts, from five different highly trained runners, we incorporated each feature across varying window lengths from the sessions \{10, 20, 30, 60, 120, 300, and 600 seconds\} to illustrate how each feature contributes to the runner's unique signature in relation to the different dynamics exhibited between HR and the other parameters.


==> Sections/oldKalmanVO2Text.tex <==


% Physiological VO$_{2}$ dynamics present unique modeling challenges: they exhibit both rapid short-term fluctuations and slower physiological adaptations, while following metabolic constraints that govern transition rates between energy states. To handle these complexities, we propose a Kalman filter–inspired deep architecture that treats VO$_{2}$ tracking as a state-estimation problem.

% Our \textit{KalmanVO2Model} ingests a 10-dimensional vector composed of seven biomechanical features, HR, positional encodings, and time-since-start. The model comprises multiple modules that jointly capture VO$_{2}$ dynamics.

% The first component involves \textbf{Feature Encoding}, where input features are processed through a multi-layer perceptron for each time step:
% \begin{equation}
% e_t = \text{MLP}(x_t; \theta_{enc}).
% \nonumber
% \end{equation} At each time step \(t\), the raw input \(x_t\) is passed through a Multilayer Perceptron (MLP) with parameters \(\theta_{\text{enc}}\). The resulting encoded vector \(e_t\) provides a learned representation that highlights important features for downstream temporal processing. Following this, \textbf{Temporal Processing} occurs, where encoded features are processed using a bidirectional GRU~\citep{chung2014empirical} to capture temporal context in both directions:
% \begin{equation}
% h_t = \text{BiGRU}(e_1, e_2, \ldots, e_T; \theta_{GRU}).
% \nonumber
% \end{equation} Here, each hidden state \(h_t\) is computed by a bidirectional GRU with parameters \(\theta_{\text{GRU}}\). 
% By processing the full sequence \(\{e_1, \ldots, e_T\}\) in both forward and backward directions, the network integrates past and future context to better capture temporal dependencies.

% The model then performs \textbf{Kalman Parameter Prediction}, deriving key filter parameters from the final hidden state:
% \begin{align}
% \sigma^2_{process} &= \text{Softplus}(\text{MLP}(h_T; \theta_{p})) + 0.1,\nonumber \\
% \sigma^2_{measurement} &= \text{Softplus}(\text{MLP}(h_T; \theta_{m})) + 0.1, \nonumber \\
% \mu_{initial} &= \text{MLP}(h_T; \theta_{\mu}) \nonumber \\
% \sigma^2_{initial} &= \text{Softplus}(\text{MLP}(h_T; \theta_{\sigma})) + 0.1, \nonumber \\
% \Delta_{max} &= \text{Softplus}(\text{MLP}(h_T; \theta_{\Delta})) + 20.0.\nonumber
% \end{align}After processing the sequence, the model derives core Kalman parameters from the final hidden state \(h_T\). These parameters govern process and measurement noise (\(\sigma^2_{\text{process}}\), 
% \(\sigma^2_{\text{measurement}}\)), initial state estimates (\(\mu_{\text{initial}}, \sigma^2_{\text{initial}}\)), 
% and the maximum allowable change \(\Delta_{\text{max}}\). In particular, \(\Delta_{\text{max}}\) enforces that state transitions remain within physiologically plausible bounds, thereby embedding essential physiological constraints directly into the Kalman filter framework.

% At the core of our approach is \textbf{Differentiable Kalman Filtering}, which performs sequential state estimation while respecting physiological constraints:
% \begin{align}
% \hat{y}_t &= \hat{y}_{t-1} + \mathcal{K}_t \cdot \text{clamp}(z_t - \hat{y}_{t-1}, -\Delta_{max}, \Delta_{max}) \nonumber\\
% \mathcal{K}_t &= \frac{P_{t|t-1}}{P_{t|t-1} + \sigma^2_{measurement}} \nonumber\\
% P_{t|t} &= (1 - \mathcal{K}_t) \cdot P_{t|t-1} \nonumber\\
% P_{t+1|t} &= P_{t|t} + \sigma^2_{process} \nonumber
% \end{align}
% Here, $\hat{y}_t$ represents the VO$_{2}$ estimate at time $t$, $z_{t}$ is the neural measurement, $\mathcal{K}_t$ is the Kalman gain, and $P_{t|t}$ represents the state variance. The $\text{clamp}$ function enforces physiological constraints by limiting state transitions to biologically plausible ranges. Unlike traditional Kalman filters that assume linear dynamics and Gaussian noise, our formulation incorporates learned metabolic constraints through $\Delta_{max}$ and adapts the measurement-state balance through learned noise parameters.

% A unique aspect of our approach is the integration of physiological constraints directly into the filter. The model learns maximum allowed VO$_{2}$ change constraints ($\Delta_{max}$) from data, effectively capturing the metabolic limitations that govern transitions between energy states. This parameter operationalizes domain knowledge that oxygen uptake cannot change arbitrarily quickly due to cardiorespiratory and muscle oxygen extraction limitations.

% \textbf{Trend Awareness and Blending.} We extend the Kalman framework with momentum-based prediction:
% \begin{equation}
% \hat{y}_{t|t-1} = \hat{y}_{t-1|t-1} + \omega \cdot (\hat{y}_{t-1|t-1} - \hat{y}_{t-2|t-2}),
% \nonumber
% \end{equation}
% where \(\omega\) is a learned weight that captures recent VO$_{2}$ velocity. We also add a blending mechanism for initial timesteps:
% \begin{equation}
% \hat{y}_t = (1 - \beta_t)\,\hat{y}_{t|t} + \beta_t\,\text{DirectNN}(h_t),
% \nonumber
% \end{equation}
% with \(\beta_t\) decreasing over the first 10 steps. This blend transitions smoothly from direct NN outputs to fully Kalman-filtered estimates, accommodating high uncertainty in early predictions.

% \subsection*{Training Methodology}
% To address the complex physiological dynamics of VO$_{2}$ during exercise, we developed a three-component loss function that progressively shifts emphasis from basic accuracy to physiological plausibility:

% \begin{equation}
% \mathcal{L}_{total} = w_{base} \cdot \mathcal{L}_{base} + w_{dynamic} \cdot \mathcal{L}_{dynamic} + w_{aux} \cdot \mathcal{L}_{auxiliary}
% \nonumber
% \end{equation}

% where $\mathcal{L}_{base}$ is the standard mean absolute error, $\mathcal{L}_{dynamic}$ captures temporal patterns, and $\mathcal{L}_{auxiliary}$ ensures physiological consistency in the predictions.

% The base loss is meant for a point-wise accuracy:
% \begin{equation}
% \mathcal{L}_{base} = \frac{1}{N} \sum_{i=1}^{N} |y_i - \hat{y}_i| \nonumber
% \end{equation}

% The dynamic loss employs a multi-step formulation that balances velocity and acceleration pattern matching:
% \begin{equation}
% \begin{split}
% \mathcal{L}_{dynamic} = \alpha \cdot \mathcal{L}_{MAE} + (1-\alpha) \cdot (0.5 \cdot \mathcal{L}_{velocity} + \\
% 0.3 \cdot \mathcal{L}_{acceleration} + 0.2 \cdot \mathcal{L}_{sign}), \nonumber
% \end{split}
% \end{equation}

% \begin{align}
% \mathcal{L}_{velocity} &= \frac{1}{N-1} \sum_{i=1}^{N-1} |(y_{i+1} - y_i) - (\hat{y}_{i+1} - \hat{y}_i)|, \nonumber\\ 
% \end{align}

% \begin{align}
% \mathcal{L}_{acceleration} &= \frac{1}{N-2} \sum_{i=1}^{N-2} |(d^2y_i - d^2\hat{y}_i)|, \nonumber \\
% \mathcal{L}_{sign} &= \text{BCE}(\text{sgn}(\hat{y}_{i+1} - \hat{y}_{i}), \mathbf{1}_{(y_{i+1} - y_{i}) > 0}),\nonumber
% \end{align}

% \noindent where $d^2y_{i} = (y_{i+2} - y_{i+1}) - (y_{i+1} - y_{i})$ represents the second-order difference. The sign matching loss specifically penalizes directional prediction errors, ensuring physiologically consistent transitions.

% For our Kalman-inspired model, the auxiliary loss encourages predicted VO$_{2}$ statistics to match empirical distributions:

% \begin{equation}
% \mathcal{L}_{auxiliary} = |\mu_{pred} - \mu_{true}| + |\sigma_{pred} - \sigma_{true}| + 0.5 \cdot |\Delta_{max} - \Delta_{true}| \nonumber
% \end{equation}

% where $\mu_{true}$ represents the mean VO$_{2}$ value, $\sigma_{true}$ its standard deviation, and $\Delta_{true}$ the 95th percentile of absolute changes between consecutive measurements.
% A key innovation in our training approach is the use of curriculum learning through dynamic weight scheduling. We gradually shift emphasis from simple to complex objectives:
% \begin{align}
% w_{base} &= \max(0.3, 1.0 - \text{epoch}/20) \nonumber\\
% w_{dynamic} &= 1.0 - w_{base} \nonumber \\
% w_{aux} &= \min(0.3, 0.1 + \text{epoch} \cdot 0.01) \nonumber
% \end{align}
% This schedule begins by prioritizing basic accuracy ($w_{base} \approx 1.0$) while gradually increasing the importance of dynamic patterns and physiological constraints. Similarly, we implement adaptive gradient clipping that relaxes as training progresses:
% $
% \text{clip\_value} = 1.0 + 4.0 \cdot e^{-\text{epoch}/10}, \nonumber
% $
% allowing larger updates early in training (clip value $\approx$ 5.0) while stabilizing later (approaching 1.0). This curriculum learning approach helps the model establish reasonable baseline predictions before refining them to capture the dynamics of VO$_{2}$ during exercise transitions.



% \subsection*{A.2 Kalman Filter Heart Rate Model}
% Our second approach treats HR prediction as a state-estimation problem using an enhanced Kalman filter. Unlike traditional implementations, we use neural networks to predict all filter parameters and employ a two-dimensional state representation that tracks both HR and its rate of change.

% We define the state vector $\mathbf{s}_t = [h_t, v_t] \in \mathbb{R}^{B \times 2}$, where $h_t$ is the HR and $v_t$ is the velocity (rate of change) of HR at time $t$. The state covariance matrix $\mathbf{P}_t \in \mathbb{R}^{B \times 2 \times 2}$ represents uncertainty in the state estimate. The process noise covariance $\mathbf{Q} \in \mathbb{R}^{B \times 2 \times 2}$ and measurement noise variance $\mathbf{R} \in \mathbb{R}^B$ are predicted by neural networks.

% As with the ODE model, we begin by processing input features through an encoder and GRU:
% \begin{align}
% \mathbf{F}_{\text{encoded}} &= f_{\text{encoder}}(\mathbf{F}_{\text{input}}) \\
% \mathbf{H} &= \text{GRU}(\mathbf{F}_{\text{encoded}})
% \end{align}

% From the final hidden state, we predict all Kalman filter parameters:
% \begin{align}
% \mathbf{Q}[:, 0, 0] &= f_{Q_{hr}}(\mathbf{H}[:, -1, :]) + 0.1 \quad \text{(Process noise for HR)} \\
% \mathbf{Q}[:, 1, 1] &= f_{Q_{vel}}(\mathbf{H}[:, -1, :]) + 0.1 \quad \text{(Process noise for velocity)} \\
% \mathbf{R} &= f_R(\mathbf{H}[:, -1, :]) + 0.1 \quad \text{(Measurement noise)}
% \end{align}

% The initial state is either provided (for HR) or predicted (for velocity):
% \begin{align}
% \mathbf{s}_0[0] &= 
% \begin{cases}
% h_0^{\text{true}} & \text{if provided} \\
% f_{init\_hr}(\mathbf{H}[:, -1, :]) & \text{otherwise}
% \end{cases} \\
% \mathbf{s}_0[1] &= f_{init\_vel}(\mathbf{H}[:, -1, :])
% \end{align}

% Similarly, we predict the initial covariance:
% \begin{align}
% \mathbf{P}_0[:, 0, 0] &= f_{P_{hr}}(\mathbf{H}[:, -1, :]) + 0.1 \\
% \mathbf{P}_0[:, 1, 1] &= f_{P_{vel}}(\mathbf{H}[:, -1, :]) + 0.1
% \end{align}

% The Kalman filter operates recursively through prediction and update steps:

% \textbf{Prediction Step:}
% In the prediction step, we use a neural network-based transition model to predict the next state:
% \begin{align}
% \mathbf{z}_t &= [\mathbf{H}[:, t, :], \mathbf{s}_t] \quad \text{(Concatenate features and state)} \\
% \Delta\mathbf{s}_t &= f_{transition}(\mathbf{z}_t) \quad \text{(State change prediction)} \\
% \mathbf{s}_{t+1}^- &= \mathbf{s}_t + \Delta\mathbf{s}_t \quad \text{(State prediction)}
% \end{align}

% This differs from traditional Kalman filters that use fixed transition matrices, allowing our model to adapt to input context. The covariance is also updated:
% \begin{align}
% \mathbf{P}_{t+1}^- &= \mathbf{P}_t + \mathbf{Q}
% \end{align}

% \textbf{Update Step:}
% For the update step, we first generate an HR observation from features:
% \begin{align}
% z_t &= f_{obs}(\mathbf{H}[:, t, :]) \nonumber
% \end{align}

% Then, we calculate the innovation (the difference between observation and prediction):
% \begin{align}
% \nu_t &= z_t - \mathbf{s}_t^-[0]
% \end{align}

% An innovation in our approach is the adaptive Kalman gain that responds to prediction errors:
% \begin{align}
% \text{base\_gain}_t &= \frac{\mathbf{P}_t^-[:, 0, 0]}{\mathbf{P}_t^-[:, 0, 0] + \mathbf{R} + 10^{-6}}
% \end{align}

% If we have error history available, we adjust the gain:
% \begin{align}
% \text{mean\_abs\_error}_t &= \frac{1}{L}\sum_{i=t-L}^{t-1}|\nu_i| \quad \text{(Over recent history)} \\
% \text{error\_factor}_t &= \sigma\left(\frac{\text{mean\_abs\_error}_t}{10.0}\right) \\
% \mathbf{K}_t[0] &= \text{clamp}\left(\text{base\_gain}_t \cdot (1 + \text{error\_factor}_t), 0.1, 0.9\right)
% \end{align}

% For the velocity component, we use a reduced gain:
% \begin{align}
% \mathbf{K}_t[1] &= \mathbf{K}_t[0] \cdot 0.5
% \end{align}

% It is a critical aspect of our model: the velocity is a hidden state not directly observed but updated through the HR innovation with a reduced gain. It is estimated and tracked to provide smoother predictions and better modeling of HR dynamics, similar to how position-velocity models improve motion tracking.

% Finally, we update the state and covariance:
% \begin{align}
% \mathbf{s}_t[0] &= \mathbf{s}_t^-[0] + \mathbf{K}_t[0] \cdot \nu_t \quad \text{(Updated HR)} \\
% \mathbf{s}_t[1] &= \mathbf{s}_t^-[1] + \mathbf{K}_t[1] \cdot \nu_t \quad \text{(Updated velocity)} \\
% \mathbf{P}_t[:, 0, 0] &= (1 - \mathbf{K}_t[0]) \cdot \mathbf{P}_t^-[:, 0, 0] \\
% \mathbf{P}_t[:, 1, 1] &= (1 - \mathbf{K}_t[1]) \cdot \mathbf{P}_t^-[:, 1, 1]
% \end{align}

% To ensure physiological plausibility, we constrain HR predictions:
% \begin{align}
% \mathbf{s}_t[0] &= \text{clamp}(\mathbf{s}_t[0], 40, 220)
% \end{align}

% Our Kalman filter approach offers several advantages: (1) The two-dimensional state vector captures both HR and its rate of change, enabling a better tracking of cardiac dynamics; (2) The adaptive Kalman gain responds to prediction errors, increasing when errors are high to give more weight to new measurements; (3) Neural network prediction of filter parameters allows adaptation to different individuals and exercise contexts; (4) The reduced gain for velocity updates creates smoother trajectories while maintaining responsiveness to intensity changes, and lastly (5) the physiological constraints ensure biologically plausible predictions.

